CubeFlow: Money Laundering Detection with Coupled Tensors

Money laundering (ML) is the behavior to conceal the source of money achieved by illegitimate activities, and always be a fast process involving frequent and chained transactions. How can we detect ML and fraudulent activity in large scale attributed transaction data (i.e.~tensors)? Most existing methods detect dense blocks in a graph or a tensor, which do not consider the fact that money are frequently transferred through middle accounts. CubeFlow proposed in this paper is a scalable, flow-based approach to spot fraud from a mass of transactions by modeling them as two coupled tensors and applying a novel multi-attribute metric which can reveal the transfer chains accurately. Extensive experiments show CubeFlow outperforms state-of-the-art baselines in ML behavior detection in both synthetic and real data.

==> Makefile <==
MAIN = EigenPulse
TEXPARTS = EigenPulse.bib \
	0-abstract.tex \
	1-introduction.tex \
	2-relatedwork.tex \
	3-method.tex \
	4-experiment.tex \
	5-conclusions.tex \
FIGURES = ./figs/*.*

all: 
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex
	open $(MAIN).pdf &
	

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) $(FIGURES)
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex
	open $(MAIN).pdf
	
clean:
	\rm -f *.aux *.bbl *.blg *.log *.thm *.out 

spotless: clean
	\rm -f $(MAIN).pdf


